KloakDB: A Platform for Analyzing Sensitive Data with $K$-anonymous Query Processing

A private data federation enables data owners to pool their information for querying without disclosing their secret tuples to one another. Here, a client queries the union of the records of all data owners. The data owners work together to answer the query using privacy-preserving algorithms that prevent them from learning unauthorized information about the inputs of their peers. Only the client, and a federation coordinator, learn the query's output. KloakDB is a private data federation that uses trusted hardware to process SQL queries over the inputs of two or more parties. Currently private data federations compute their queries fully-obliviously, guaranteeing that no information is revealed about the sensitive inputs of a data owner to their peers by observing the query's instruction traces and memory access patterns. Oblivious querying almost always exacts multiple orders of magnitude slowdown in query runtimes compared to plaintext execution, making it impractical for many applications. KloakDB offers a semi-oblivious computing framework, $k$-anonymous query processing. We make the query's observable transcript $k$-anonymous because it is a popular standard for data release in many domains including medicine, educational research, and government data. KloakDB's queries run such that each data owner may deduce information about no fewer than $k$ individuals in the data of their peers. In addition, stakeholders set $k$, creating a novel trade-off between privacy and performance. Our results show that KloakDB enjoys speedups of up to $117$X using k-anonymous query processing over full-oblivious evaluation.

==> plots/query2/query2.tex <==
    \begin{tikzpicture}
\begin{axis}[
    scale=.75,
    yscale=.75,
        ymin=1,
    xscale=.92,
    area legend,
ylabel={Execution Time (ms)},
    legend style={at={(0.21,1.65)},
      anchor=north,legend columns=-1, draw=none},
    xlabel={$k$ parameter},
    symbolic x coords={1,10,20,30,40,50,60,70,80,90,100},
    xtick=data,
    ticklabel style = {font=\scriptsize},
    ylabel near ticks, yticklabel pos=left,
    /pgf/number format/1000 sep={},
    axis x line*=bottom
    ]
    %encrypted runtimes
	\addplot[mark=triangle,line legend, thick, sharp plot, stack plots=false,  point meta=rawy] coordinates {(1,40) (10,90) (20,154) (30, 202) (40, 274) 
			 (50,321) (60,380) (70, 441) (80, 498) (90, 557) (100, 600)};
			     

    \addlegendentry{Runtime}
\end{axis}
\begin{axis}[
    scale=.75,
    yscale=.75,
    xscale=.92,
    area legend,
    axis x line*=bottom,
    ybar,
        ymin=1,
    legend style={at={(0.8,1.65)},
      anchor=north,legend columns=-1, draw=none},
    ylabel near ticks, yticklabel pos=right,
    ylabel={Output Tuples},
    ylabel style={rotate=180},
    xtick pos=left,
    bar width=.55em,
    symbolic x coords={1,10,20,30,40,50,60,70,80,90,100},
    xticklabels={,,},
    ]
	    %\addplot[black, fill=gray] coordinates {(1,88618) (10,287232) (20,544730) (30, 795890) (40, 1032050) 
	%		 (50,1310520) (60,1543230) (70, 1800982) (80, 2067382) (90, 2312088) (100, 2553722)};
	    \addplot[draw=black, fill=black] coordinates {(1,88.618) (10,287.232) (20,544.730) (30, 795.890) (40, 1032.050) 
			 (50,1310.520) (60,1543.230) (70, 1800.982) (80, 2067.382) (90, 2312.088) (100, 2553.722)};

    \addlegendentry{Tuple Count}
\end{axis}
    \end{tikzpicture}


==> plots/query3/query3.tex <==

    \begin{tikzpicture}
\begin{axis}[
    yscale=.58,
		xscale=.75,
	ybar,
    ymin=0,ymax=40000,
    enlargelimits=0.15,
    legend style={at={(0.534,2.2)},
      anchor=north,legend columns=4, legend style={draw=none}
      },
	ylabel={Execution Time (ms)},
    xlabel={Input Tuples },
    bar width=.65em,
    ylabel near ticks, 
    ymode=log,
    area legend,
    log basis y=10,
    axis y line*=left,
    axis x line*=bottom,
    symbolic x coords={$10^3$,$10^4$,$10^5$,$10^6$,$10^7$},
    xtick=data,
    ytick pos=left,
    xtick pos=left,
    x label style={at={(axis description cs:.53,0.28)}, anchor=north},
    ]
	    %\addplot [draw=gray, fill=gray] coordinates {($10^2$,4.11) ($10^3$,3.37) ($10^4$,7.56) ($10^5$, 30.04) 
%							($10^6$, 298.03) ($10^7$, 20359.60)};
	    \addplot [pattern=north west lines] coordinates {($10^3$, 76.68) ($10^4$,73.993) ($10^5$, 130.5518) ($10^6$, 853.08) ($10^7$, 8113.362)};
	    \addplot [draw=black, fill=black] coordinates { ($10^3$,50.78) ($10^4$,56.925) ($10^5$, 162.0982) ($10^6$, 1131.498) ($10^7$, 10721.0)};
	    \addplot[mark=triangle,line legend, thick, sharp plot, stack plots=false] coordinates { ($10^3$,127.25) ($10^4$,133.815) ($10^5$, 314.5628) ($10^6$, 2081.228) ($10^7$,19458.86)};

  %  \addlegendentry{hello}
%    \legend{rand., shuffle, hash, sort, redist., total}
    \legend{Unlink, Repart., Total}
\end{axis}
    \end{tikzpicture}
	    %\addplot coordinates {(1,4000) (10,51958) (20,91956) (30, 175834) (40, 175834) 
	%		 (50,231886) (60,275864) (70, 307702) (80, 347828) (90, 457702) (100, 470706)};


==> plots/query5/query5_exec_time.tex <==
\begin{tikzpicture}
\begin{axis}[
    yscale=.73,
    xscale=.73,
    ybar stacked,
    enlargelimits=0.15,
    legend style={at={(.68,1.5)},
      anchor=north,legend columns=4, draw=none, font=\small},
    symbolic x coords={enc.,5,10,15,20},
ylabel={Execution Time (ms)},
    ymin=0,
    ymode=log,
    log basis y=10,
    xtick=data,
    x label style={at={(axis description cs:.61,0)}, anchor=north},
    xlabel={$k$ parameter},
    area legend,
    bar width=1em,
    axis y line*=left,
    axis x line*=bottom,
    ytick pos=left,
    xtick pos=left
    ]
    %encrypted runtimes
    	\addplot+[ybar, draw=black, preaction={fill=lightgray}, pattern=dots] plot coordinates {(enc.,2.7) (5,2.6) (10,2.6) (15,2.8) (20,3.5)};https://www.overleaf.com/project/5b10574851d0dc20dac4c320
	\addplot+[ybar, draw=teal, preaction={fill=teal}, pattern=north west lines, opacity=.9] plot coordinates {(enc.,3.26) (5,3.8) (10,5.49) (15,10.8) (20,23.4)};
	\addplot+[ybar, draw=darkgray, preaction={fill=white}, pattern=crosshatch, opacity=1] plot coordinates {(enc.,3.1) (5,13.2) (10,39.9) (15,90.7) (20,303)};
    	\addplot+[ybar, draw=black, fill=black] plot coordinates {(enc.,3.38) (5,48.4) (10,296) (15,1629) (20,8125)};
	\legend{ Join 1\,\,,Join 2\,\,, Join 3\,\,,Join 4}%obliv.}
\end{axis}
\end{tikzpicture}

%Oblivious
%4: 241.865 Seconds
%3: 9.0199
%2: .268441
%1: .110552

%K=18
%4: 237.779 (gen level 5)
%3: 5.8275 (gen level 5)
%2: .542622 (gen level 5)
%1: .089643 (gen level 5)


%K=10
%4: 30.0459 (gen level 4)
%3: 1.18699 (gen level 4)
%2: .222832 (gen level 4)
%1: .063146 (gen level 4)

%K=5
%4: 8.51486 (gen level 3)
%3: .483357 (gen level 3)
%2: .173168 (gen level 3)
%1: .088408 (gen level 3)

%K=2
%4: .520455 (gen level 1)
%3: .241431 (gen level 1)
%2: .098356 (gen level 1)
%1: .05325 (gen level 1)

%Encrypted
%4: .300477
%3: .142628
%1: .130762
%1: .038094



==> plots/query7/query7_asp.tex <==
\begin{tikzpicture}
\begin{axis}[
    ybar,
    yscale=.6,
    enlargelimits=0.15,
	legend pos = south west,
	legend style={at={(0,1.55)},legend columns=4},
    ylabel={Execution Time (ms)},
    xlabel={Query},
    symbolic x coords={Aspirin Profile},
    ymode=log,
    log basis y=10,
    xtick=data,
    bar width=1em,
    ytick pos=left,
    xtick pos=left
    ]
    %COLLOCATED, POSTGRES
	\addplot [pattern=crosshatch] coordinates {(Aspirin Profile,1)}; %FDW single host, timing end to end
	\addplot [pattern=dots] coordinates {(Aspirin Profile, 250.270333333)}; %ENCRYPTED IN VAULTDB
	\addplot [pattern=north west lines] coordinates {(Aspirin Profile, 10575.07875)}; %5-anon IN VAULTDB
	\addplot [draw=black, fill=black] coordinates {(Aspirin Profile, 93513.9)}; %OBLIVIOUS
    \legend{FDW,encrypted, 5-anon, oblivious}
\end{axis}
\end{tikzpicture}


==> plots/query8/query8-linear-axis.tex <==
\begin{tikzpicture}
	\begin{axis}[ybar stacked,enlargelimits=0.25, bar shift=-12pt, xticklabels={}, yticklabels={}]
% Stats Collection
	\addplot coordinates
    		{(1,757) (2,763) (3,789.9)  };
    % KPV generation
	\addplot coordinates
		{(1,535.5) (2,556.5) (3,752) };	
	\addplot coordinates
	{(1,215) (2,234.8) (3,580) };		
		
\end{axis}


	\begin{axis}[ybar stacked,enlargelimits=0.25, bar shift=0pt, xticklabels={}, yticklabels={}]
% Stats Collection
	\addplot coordinates
    		{ (1,758) (2,790.2) (3,833) };
    % KPV generation
	\addplot coordinates
		{ (1,584.7) (2,670) (3,819) };	
	\addplot coordinates
		{(1,215.3) (2,234) (3,568) };		
		
\end{axis}


% 100k tuples
	\begin{axis}[ybar stacked,enlargelimits=0.25, bar shift=12pt, xticklabels={}, yticklabels={}]
% Stats Collection
	\addplot coordinates
    		{ (1,762) (2,802) (3,3839) };
    % KPV generation
	\addplot coordinates
		{ (1,601) (2,1736) (3,2995) };	
	\addplot coordinates
		{ (1,208) (2,203.8) (3,553) };		
		
\end{axis}

\end{tikzpicture}


==> plots/query8/query8.tex <==
%\documentclass{article}
%\usepackage{tikz}
%\usepackage{pgfplots}

%\usetikzlibrary{arrows}
%\usetikzlibrary{shapes.geometric,positioning}
%\usetikzlibrary{patterns}
%\usetikzlibrary{snakes}
%\begin{document}
\begin{tikzpicture}[
		every axis/.style={
    ybar stacked,
    yscale=.53,
    xscale=.65,
	bar width=15pt,
    enlargelimits=0.15,
    ymin=1100, ymax=8000,
    %ymode=log,
    %log basis y=10,
    axis y line*=left,
    axis x line*=bottom,
    legend style={at={(0.789,2.12)},
      anchor=north,legend columns=3, draw=none},
	symbolic x coords={1000, 10000, 100000},
    xtick=data,
    scaled ticks = false,
	tick label style={/pgf/number format/fixed},
	x tick label style={rotate=0,yshift={-.22em}},
			},
		]
			\node at (-.80,3.79) {\textit{\# Tuples:}};
		\pgfplotsset{
			% define a new style used for the plot used to add labels
			% 2 args means it takes two mandatory arguments, so must be used as
			% labelplot={first arg}{second arg}
			labelplot/.style 2 args={
				% forget plot means it doesn't affect cycle lists or legends
				forget plot,
				% #1 is first argument, the text used in the nodes near coords
				nodes near coords=#1,
				% #2 is second argument, a length that should be the same as the bar shift for the axis
				every node near coord/.style={below,font=\tiny,xshift=#2}
				}
				}

				\begin{axis}[bar shift=-15pt, xticklabels={}, yticklabels={}]
				%range 1k, stats
	\addplot+[ybar,fill=lightgray, draw=black] plot coordinates {(1000,757) (10000,758) (100000, 762.2)};
	
\addplot+[ybar, preaction={fill=lightgray},draw=black,pattern=dots, draw=black, opacity=.2] plot coordinates {(1000, 535.5)  (10000,584.7) (100000,601)};

\addplot+[ybar, draw=black,pattern=crosshatch, preaction={fill=lightgray}, draw=black, opacity=.9] plot coordinates {(1000,215) (10000,215.3) (100000,208.0)};
\legend{\strut Stats.\,\,, \strut KPV Gen.\,\,, \strut Redist.}
				\end{axis}
	\begin{axis}[bar shift=-15pt, xticklabels={}, yticklabels={},
    legend style={at={(.162,2.43)},
			anchor=north,legend columns=3}]

	\addplot+[ybar,fill=lightgray, draw=black] plot coordinates {(1000,757) (10000,758) (100000, 762.2)};
	
\addplot+[ybar, preaction={fill=lightgray},draw=black,pattern=dots, draw=black, opacity=.2] plot coordinates {(1000, 535.5)  (10000,584.7) (100000,601)};

\addplot+[ybar, draw=black,pattern=crosshatch, preaction={fill=lightgray}, draw=black, opacity=.9] plot coordinates {(1000,215) (10000,215.3) (100000,208.0)};

			\addlegendentry{1000}
\end{axis}

	\begin{axis}[xticklabels={$1\cdots10^3$, $1\cdots10^4$, $1\cdots10^5$},
    xticklabel style={text width=3em, rotate=0},
		xlabel={Range of Input Domain}, ylabel={Execution Time (ms)}, x label style={at={(axis description cs:.7,0)}, anchor=north},
y label style={at={(axis description cs:-.22,1.0)}, anchor=north},
    legend style={at={(.59,2.43)},
			anchor=north,legend columns=3}]
	        %stats, all tuple sizes, 10k range
			\addplot+[ybar,fill=brown, draw=black] plot coordinates {(1000,763) (10000,790.2) (100000, 802.9)};
			\addlegendentry{10000}
			%KPV gen, 10k range
			\addplot+[ybar, preaction={fill=brown},draw=brown,pattern=dots, draw=black, opacity=.2] plot coordinates {(1000,556.5) (10000,670) (100000,1736.2)};
			\addplot+[ybar, draw=black,pattern=crosshatch, preaction={fill=brown}, draw=black, opacity=.9] plot coordinates {(1000,234.8) (10000,234) (100000,203)};
\end{axis}

	\begin{axis}[bar shift=15pt, xticklabels={}, yticklabels={},
    legend style={at={(1.089,2.42)},
			anchor=north,legend columns=3}]

	\addplot+[ybar,fill=darkgray, draw=black] plot coordinates {(1000,798.9) (10000,830.2) (100000, 3839)};
			\addlegendentry{100000}
\addplot+[ybar, preaction={fill=darkgray},draw=darkgray,pattern=dots, draw=black, opacity=.2] plot coordinates { (1000,752.4) (10000,823.2) (100000, 2995)};
\addplot+[ybar, draw=black,pattern=crosshatch, preaction={fill=darkgray}, draw=black, opacity=.9] plot coordinates { (1000,580) (10000,563.3) (100000, 553)};
	\end{axis}
\end{tikzpicture}
%\end{document}


==> plots/query9_agg/query8-linear-axis.tex <==
\begin{tikzpicture}
	\begin{axis}[ybar stacked,enlargelimits=0.25, bar shift=-12pt, xticklabels={}, yticklabels={}]
% Stats Collection
	\addplot coordinates
    		{(1,757) (2,763) (3,789.9)  };
    % KPV generation
	\addplot coordinates
		{(1,535.5) (2,556.5) (3,752) };	
	\addplot coordinates
	{(1,215) (2,234.8) (3,580) };		
		
\end{axis}


	\begin{axis}[ybar stacked,enlargelimits=0.25, bar shift=0pt, xticklabels={}, yticklabels={}]
% Stats Collection
	\addplot coordinates
    		{ (1,758) (2,790.2) (3,833) };
    % KPV generation
	\addplot coordinates
		{ (1,584.7) (2,670) (3,819) };	
	\addplot coordinates
		{(1,215.3) (2,234) (3,568) };		
		
\end{axis}


% 100k tuples
	\begin{axis}[ybar stacked,enlargelimits=0.25, bar shift=12pt, xticklabels={}, yticklabels={}]
% Stats Collection
	\addplot coordinates
    		{ (1,762) (2,802) (3,3839) };
    % KPV generation
	\addplot coordinates
		{ (1,601) (2,1736) (3,2995) };	
	\addplot coordinates
		{ (1,208) (2,203.8) (3,553) };		
		
\end{axis}

\end{tikzpicture}


==> plots/query9_agg/query_agg_two_host.tex <==
%\documentclass{article}
%\usepackage{tikz}
%\usepackage{pgfplots}

%\usetikzlibrary{arrows}
%\usetikzlibrary{shapes.geometric,positioning}
%\usetikzlibrary{patterns}
%\usetikzlibrary{snakes}
%%\begin{document}
\begin{tikzpicture}
 \begin{axis}[
        xlabel=$k$ parameter,
	 ylabel=Execution Time $(ms)$,
	ymode=log,
    ytick pos=left,
    xtick pos=left,
    axis y line*=left,
    axis x line*=bottom,
	 legend style={at={(.35, 1.1)}, anchor=north,legend columns=2, draw=none}
	 ]
    \addplot[smooth,mark=*,blue] plot coordinates {
        (5,2381)
        (10,2599)
        (15,2654)
        (20,1)
    };
    \addlegendentry{Enclave}

    \addplot[smooth,color=red,mark=x]
        plot coordinates {
        (0,2)
        (5,3)
        (10,100)
        (15,100)
        (20,100)
        };
    \addlegendentry{MPC}
    \end{axis}
\end{tikzpicture}
%\end{document}


==> plots/query9_agg/query_filter_two_host.tex <==
\begin{tikzpicture}
 \begin{axis}[
        xlabel=$k$ parameter,
	 ylabel=Execution Time $(ms)$,
	ymode=log,
    ytick pos=left,
    xtick pos=left,
    axis y line*=left,
    axis x line*=bottom,
	 legend style={at={(.35, 1.1)}, anchor=north,legend columns=2, draw=none}
	 ]
    \addplot[smooth,mark=*,blue] plot coordinates {
        (0,2)
        (5,3)
        (10,1)
        (15,1)
        (20,1)
    };
    \addlegendentry{Enclave}

    \addplot[smooth,color=red,mark=x]
        plot coordinates {
        (0,2)
        (5,3)
        (10,100)
        (15,100)
        (20,100)
        };
    \addlegendentry{MPC}
    \end{axis}
\end{tikzpicture}


==> plots/query9_agg/query_sort_two_host.tex <==
\begin{tikzpicture}
 \begin{axis}[
        xlabel=$k$ parameter,
	 ylabel=Execution Time $(ms)$,
	ymode=log,
    ytick pos=left,
    xtick pos=left,
    axis y line*=left,
    axis x line*=bottom,
	 legend style={at={(.35, 1.1)}, anchor=north,legend columns=2, draw=none}
	 ]
    \addplot[smooth,mark=*,blue] plot coordinates {
        (0,2)
        (5,3)
        (10,1)
        (15,1)
        (20,1)
    };
    \addlegendentry{Enclave}

    \addplot[smooth,color=red,mark=x]
        plot coordinates {
        (0,2)
        (5,3)
        (10,100)
        (15,100)
        (20,100)
        };
    \addlegendentry{MPC}
    \end{axis}
\end{tikzpicture}

